Peripheral-free Device Pairing by Randomly Switching Power

The popularity of Internet-of-Things (IoT) comes with security concerns. Attacks against wireless communication venues of IoT (e.g., Man-in-the-Middle attacks) have grown at an alarming rate over the past decade. Pairing, which allows the establishment of the secure communicating channels for IoT devices without a prior relationship, is thus a paramount capability. Existing secure pairing protocols require auxiliary equipment/peripheral (e.g., displays, speakers and sensors) to achieve authentication, which is unacceptable for low-priced devices such as smart lamps. This paper studies how to design a peripheral-free secure pairing protocol. Concretely, we design the protocol, termed SwitchPairing, via out-of-box power supplying chargers and on-board clocks, achieving security and economics at the same time. When a user wants to pair two or more devices, he/she connects the pairing devices to the same power source, and presses/releases the switch on/off button several times. Then, the press and release timing can be used to derive symmetric keys. We implement a prototype via two CC2640R2F development boards from Texas Instruments (TI) due to its prevalence. Extensive experiments and user studies are also conducted to benchmark our protocol in terms of efficiency and security.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> Sections/sec-availability.tex <==
\section*{Availability}

The code for our BLESS tool is available at:
\\

 




==> Sections/trashbin/sec1-introduction.tex <==

\section{Introduction}

Internet of Things (IoT) has quite deservedly received a lot of recent attentions, featuring various applications, such as smart home, smart city and so forth. As a vital wireless communication media of IoT, Bluetooth Low Energy (BLE) has been adopted by a variety of these IoT applications due to its large coverage and energy-saving features, which provides a better support for the connectivity of IoT devices. As ABI Research predicts, the shipments of BLE devices will surpass 400 million by the end of 2020 \cite{ABI}.

However, the security issue is one of the gigantic barriers to the deployment of BLE-enabled applications. Various attacks on BLE have been reported, such as Man-in-the-Middle (MITM) attacks\cite{MITMJustworks} and spoofing attacks. To counter these attacks, BLE provides a set of pairing strategies for two devices to negotiate a common communication key. These pairing strategies includes {\em Just Works}, {\em Passkey-entry}, {\em Numeric Comparison} and {\em Out of band} ({\em OOB}). Among these four Pairing strategies, {\em Passkey-entry}, {\em Numeric Comparison} and  {\em OOB} are considered as secure pairing strategies, while the  {\em Just Works} is subject to MITM attacks. 

The secure pairing strategies ({\em Passkey-entry}, {\em Numeric Comparison} and {\em Out of band} ) are secure because they use a trustworthy third-party (e.g. the user or an external secure channel) to guarantee the key negotiated on both devices are the same. To this end, the two devices have to exchange security parameters that will be involved in the key generation process. That is, only when each device obtains the same security parameter from its peer device, can a same communication key be negotiated on both sides. 
To achieve this goal securely, the two devices have to exchange the security parameters via the user or an external secure channel.
For example, in {\em Passkey-entry} pairing strategy, one device display a 6 digits pin (i.e. security parameters), while the pairing operator (usually,pairing operator is the owner of the device) sees the pin, and enters the pin to another device.  In the {\em Numeric Comparison} pairing strategy, the owner has to check if pins displaying on the two pairing devices are the same and make confirmation by pressing the ''YES'' buttons on both devices. In {\em OOB}, the two pairing devices exchange the security parameters by using a secure out of band channel.  The out of band channel can be Near Field Communication (NFC), which is considered capable of defending MITM attack.  In the {\em Just Works}, the two devices exchange security parameters directly without the involvement of the user or the secure channel. Therefore, there is no way to ensure that the negotiated key are the same.   

Paring strategies are not omnipotent since it only gives a trade-off between security and economics. That is, manufacturer have to pay extra cost to guarantee the security of their products. For example, {\em Passkey-entry} or {\em Numeric Comparison} requires one device or the two devices equip displays or keypads, while {\em OOB} requires both of the two devices integrate out of band communication modules, such as NFC modules. Given the extra cost of using secure pairing strategies, the manufacturer may want to use {\em Just Works}. The fact that using the {\em Just Works} rather than the secure pairing strategies has grave impacts given BLE’s broad application domains, since the products are prone to MITM attacks. 

%A few effects have been taken to reduce the extra cost, such as 
This paper studies how to design a BLE pairing strategy that requires no extra cost for BLE devices, allowing devices to achieve security and economics simultaneously.
Our insights is that to achieve the secure pairing, the owner of the two devices needs to assist the two pairing devices to exchange security parameters securely. Therefore,  extra components are involved, such as a display or a keypad. With keyboard or display enabled on the pairing devices, even an attacker is presented, he can not eavesdrop the user's input, so that the security of the pairing process is guaranteed. %However, 
%However, is there any out of box components that can make this happen? how can security parameters be exchanged securely between two devices without involve extra components ?
\textit{Designing a secure protocol for Bluetooth Low Energy without extra cost now collapse to a question that how to exchange the security parameters  between two devices without extra communication venue.} This is a comprehensive view of BLE pairing protocols.
 

Motivated by our observation, we carefully investigate the procedure of BLE secure pairing protocol to confirm our insight.  
According to our theory, there are three requirements when designing a secure pairing protocol. (i) the two pairing devices may need to exchange security parameters via channels other than the Bluetooth channel. (ii) To the security concerns, the channel should avoid eavesdropping attack innately.  
(iii) The exchanged security parameters must be strong enough to thwart the guessing attack. The above three concerns are also the challenges we need to overcome.  


Particularly, we proposed a new pairing protocols, \texttt{Secure Just Works}, for these devices without any input/output capabilities. 
we use the power supply charger to build an alternative channel, so that they can exchange the security parameters. Using the out-of-box components will keep our design economically viable, since the most of devices have a power supply charger. (\textbf{addresses challenge (i)}) Basically, our pairing protocol works as follows: (i) the two paring devices synchronize clock frequencies via the BLE channel first.  Afterwards, the owner of the two devices switch the power source on and off intentionally for several times. We let the two devices record the time points of power switch off/on respectively. The time points are the initial values which can be used to derive a same encryption key. Obviously, in our pairing protocol, the attacker can not obtain the time points of power switch off/on (\textbf{addresses challenge (ii)}). 
Moreover, the exchanged security parameters can be very strong depending on the precision of clock and the times that user switches on/off the plug (\textbf{addresses challenge (iii)}). Please note that the power supply charger in our paper is used to demonstrate the principles, while other components that have such features can also be used to build pairing protocols. 
 

\textbf{Contributions}: We summarize the main contributions of this paper as follows:

\begin{enumerate}
\item We show that with the weak pairing protocol (Just Works) enabled, an attacker can deploy man-in-the-middle attack trivially, which grave hinder the security of Bluetooth Low Energy. A real world product has been exploited to demonstrate how the attack can be end-to-end. 
\item 
 We explore the essence of secure pairing, and summarized the features of Bluetooth pairing protocols. This is a comprehensive view of BLE pairing protocols.% \red{It is worthy note that the summarized features can also be used to design various other secure pairing protocols.} 
\item To confirm our insights, we design a new pairing protocol, termed \texttt{Secure Just works}, in which the two pairing device can negotiated a same security key without any extra input/output devices (such as Keyboard or Display). To the best of our knowledge, we are the first to trade off the economic cost and security on Bluetooth pairing. Our design provide a good guidelines for community to follow, in terms of designing secure pairing protocols.   
\item We implement a prototype via two CC2640R2F developing boards from Texas Instruments (TI) due to the prevalence of their products and the support of Bluetooth Low Energy programming framework. The source code of our prototype can be publicly accessed at \red{URL} , so that the community can benefit from our design in a timely manner. 
\item Extensive evaluations and security analysis have been preformed to benchmark our protocol. We conclude that our new protocol can also achieve high security with little overloads. 
 
 
\end{enumerate}

Particularly, we have reported our design to Bluetooth Special Interest Group (SIG), and advocate them to adopt our proposed pairing protocol. \red{They are now working with us actively to discuss the details. }

\textbf{Roadmap}:   The rest of this paper is organized as follows. 
Section \ref{sec:ble} provides the necessary background information of Bluetooth Low Energy. In Section \ref{sec:example}, we provide our threat mode and give our motivation examples. 
Section \ref{sec:implementation} presents the our Secure Just Works and its implementation criteria . Evaluations and User Studies are presented in Section \ref{sec:eva}.   Section \ref{sec:disuss} discusses a few interesting topics. Related work is presented in Section \ref{{sec:relatedwork}}. This paper is concluded in Section \ref{chap::conclusions}.


%public key and 
 

%To evaluate the security and other metrics, we perform security analysis and conduct a set of experiment afterwards. 
.  
%





 


 
